KLDrive: Fine-Grained 3D Scene Reasoning for Autonomous Driving based on Knowledge Graph

Autonomous driving requires reliable reasoning over fine-grained 3D scene facts. Fine-grained question answering over multi-modal driving observations provides a natural way to evaluate this capability, yet existing perception pipelines and driving-oriented large language model (LLM) methods still suffer from unreliable scene facts, hallucinations, opaque reasoning, and heavy reliance on task-specific training. We present KLDrive, the first knowledge-graph-augmented LLM reasoning framework for fine-grained question answering in autonomous driving. KLDrive addresses this problem through designing two tightly coupled components: an energy-based scene fact construction module that consolidates multi-source evidence into a reliable scene knowledge graph, and an LLM agent that performs fact-grounded reasoning over a constrained action space under explicit structural constraints. By combining structured prompting with few-shot in-context exemplars, the framework adapts to diverse reasoning tasks without heavy task-specific fine-tuning. Experiments on two large-scale autonomous-driving QA benchmarks show that KLDrive outperforms prior state-of-the-art methods, achieving the best overall accuracy of 65.04% on NuScenes-QA and the best SPICE score of 42.45 on GVQA. On counting, the most challenging factual reasoning task, it improves over the strongest baseline by 46.01 percentage points, demonstrating substantially reduced hallucinations and the benefit of coupling reliable scene fact construction with explicit reasoning.

==> 6.Tooldesign.tex <==

\clearpage
\section{\red{Updated all:} General Tool Design for Scene Reasoning}
\label{sec:scene-tools}

Given the scene KG $\mathcal{G}_t$ constructed in Section~\ref{sec:perception}, the remaining challenge is to let an LLM reason about the scene in a way that is both expressive and faithful to the underlying 3D world. Rather than exposing raw graph structures or continuous geometry directly to the LLM, {\systemname} introduces a small set of scene tools that mediate all interactions with $\mathcal{G}_t$. These tools are designed to be deterministic, compositional, and schema-constrained, so that the LLM’s reasoning chain becomes a grounded program over the scene graph instead of free-form, potentially hallucinated text.


%%%%%%%%%%%%%%%%
\subsection{Tool Design over the Scene Graph}
\label{subsec:atomic-ops}
We formalize scene reasoning over $\mathcal{G}_t$ as computation on \emph{sets of entities}. 
Unlike free-form traversal, the resulting operators are deterministic functions of $\mathcal{G}_t$, preventing the hallucination of non-existent entities and keeping all reasoning steps within a finite, canonical label space.
Let $\mathcal{C}$ and $\mathcal{S}$ denote the finite sets of object categories (e.g., \texttt{car}, \texttt{pedestrian}) and statuses (e.g., \texttt{moving}, \texttt{standing}), respectively. 
Each node $v_i \in \mathcal{V}_t$ is annotated with $(c_i, s_i, \mathbf{p}_i)$, where $c_i \in \mathcal{C}$, $s_i \in \mathcal{S}$, and $\mathbf{p}_i \in \mathbb{R}^2$ is its ground-plane position. 
We define a node filter $\pi$ as a Boolean predicate over node attributes (e.g., ``$c_i = \texttt{car} \wedge s_i = \texttt{moving}$''), serving as the fundamental primitive for selecting entity subsets.

\textbf{Entity Resolution.}
Entity resolution maps a linguistic object description to an explicit subset of $\mathcal{V}_t$. 
Given a node filter $\pi$, we define
\begin{equation*}
    \mathcal{V}(\pi) = \{ v_i \in \mathcal{V}_t \mid \pi(v_i) \}.
\label{eq:entity_resolution}
\end{equation*}
The resolved set $\mathcal{V}(\pi)$ serves as the basic intermediate state for subsequent reasoning. 
By resolving object descriptions into explicit subsets of $\mathcal{V}_t$, the algebra ensures that all downstream operations remain grounded in entities supported by $\mathcal{G}_t$, rather than unconstrained entities inferred directly from natural language.


\textbf{Relational Restriction.}
To support spatially conditioned queries, we define \textsf{RelSelect} under ego-centric spatial semantics. Let $\mathbf{d}_{\mathrm{ego}} \in \mathbb{R}^2$ denote the ego heading vector. For a reference node $v_{\mathrm{ref}}$ and a candidate node $v_j$ with ground-plane positions $\mathbf{p}_{\mathrm{ref}}$ and $\mathbf{p}_j$, respectively, we first compute the relative displacement and signed angle:
\begin{equation*}
\begin{aligned}
    \mathbf{d}_{\mathrm{ref},j} &= \mathbf{p}_j - \mathbf{p}_{\mathrm{ref}},\\
    \theta_{\mathrm{ref},j} &= \angle_{\mathrm{signed}}(\mathbf{d}_{\mathrm{ref},j}, \mathbf{d}_{\mathrm{ego}}) \in (-\pi,\pi].
\end{aligned}
\end{equation*}
We then quantize $\theta_{\mathrm{ref},j}$ into a finite ego-centric relation vocabulary $\mathcal{R}$ via
$\Phi_{\mathrm{angle}} : (-\pi,\pi] \rightarrow \mathcal{R}$, and define
$r=\Phi_{\mathrm{angle}}(\theta_{\mathrm{ref},j}) \in \mathcal{R}$.
In practice,
$\mathcal{R}=\{\texttt{front}$, $\texttt{front\_left}$, $\texttt{back\_left}$,$\texttt{back}$,$\texttt{back\_right}$,$\texttt{front\_right}\}$, with angular boundaries at $\pm30^\circ$, $\pm90^\circ$, and $\pm150^\circ$. 
The sectorization is designed to be consistent with the qualitative spatial relations used in the QA dataset~\cite{qian2024nuscenes}, so that language-level directional expressions can be mapped to a deterministic geometric interpretation.
Accordingly, the relation predicate $\rho_r(v_{\mathrm{ref}},v_j)$ holds when $\Phi_{\mathrm{angle}}(\theta_{\mathrm{ref},j})=r$, and the reference-conditioned candidate set is
\begin{equation*}
\begin{gathered}
\mathcal{V}_r(v_{\mathrm{ref}},\pi)
=
\{\, v_j \in \mathcal{V}_t \mid \pi(v_j)\wedge \rho_r(v_{\mathrm{ref}},v_j)\,\},\\
\textsf{RelSelect}(v_{\mathrm{ref}},r,\pi)
=
\operatorname{Sort}_{d(\cdot, v_{\mathrm{ref}})}\!\big(\mathcal{V}_r(v_{\mathrm{ref}},\pi)\big).
\end{gathered}
\end{equation*}
Under this design, the reference object serves only as an anchor point, while directional semantics are interpreted globally in the ego frame rather than in the object's local frame. We retain only directional predicates and map natural-language spatial descriptions to precise, executable relation tokens. 
Moreover, \textsf{RelSelect} returns candidates in nearest-first order, so that expressions such as ``the car in front of the pedestrian'' are deterministically resolved to the nearest valid instance.

\textbf{Set Composition and Query.}
More complex questions are expressed by composing intermediate entity sets and applying typed queries to the resulting subsets. 
We first define the basic set operations and cardinality queries:
\begin{equation*}
\begin{aligned}
    \textsf{Intersect}(\mathcal{V}_A, \mathcal{V}_B) &= \mathcal{V}_A \cap \mathcal{V}_B,\\
    \textsf{Count}(\mathcal{V}') &= |\mathcal{V}'|,\\
    \textsf{Exists}(\mathcal{V}') &= \mathbb{I}[\,\mathcal{V}' \neq \emptyset\,].
\end{aligned}
\label{eq:set_queries}
\end{equation*}
We then define typed queries over the selected subsets:
\begin{equation*}
    \textsf{SameStatus}(\mathcal{V}_A, \mathcal{V}_B) \in \{\texttt{yes}, \texttt{no}\}.
\label{eq:same_status}
\end{equation*}
\begin{equation*}
    \textsf{GetType}(\mathcal{V}') \in \mathcal{C}, \qquad
    \textsf{GetStatus}(\mathcal{V}') \in \mathcal{S}.
\label{eq:get_fields}
\end{equation*}
Here, $\textsf{Intersect}$ composes resolved subsets under multiple constraints, $\textsf{Count}$ and $\textsf{Exists}$ query the cardinality and non-emptiness of the resulting set, and $\textsf{SameStatus}$ performs typed comparison across subsets. 
For attribute queries, $\textsf{GetType}$ and $\textsf{GetStatus}$ return a single canonical label for $\mathcal{V}'$ via a deterministic representative rule.
Together, these operators decompose fine-grained scene queries into explicit operations over scene-grounded entity sets. 
For example, \emph{``How many cars are in front of the standing pedestrian?''} is expressed as $\textsf{Count}(\textsf{RelSelect}(v_{\mathrm{ped}}, \texttt{front}, \pi_{\mathrm{car}}))$, where $v_{\mathrm{ped}}$ denotes the node obtained by a preceding entity-resolution step.









